Shared Memory-contention-aware Concurrent DNN Execution for Diversely Heterogeneous System-on-Chips

Two distinguishing features of state-of-the-art mobile and autonomous systems are 1) there are often multiple workloads, mainly deep neural network (DNN) inference, running concurrently and continuously; and 2) they operate on shared memory system-on-chips (SoC) that embed heterogeneous accelerators tailored for specific operations. State-of-the-art lacks efficient performance and resource management techniques necessary to either maximize total system throughput or minimize end-to-end workload latency. In this work, we propose HaX-CoNN, a novel scheme that characterizes and maps layers in concurrently executing DNN inference workloads to a diverse set of accelerators within a SoC. Our scheme uniquely takes per-layer execution characteristics, shared memory (SM) contention, and inter-accelerator transitions into account to find optimal schedules. We evaluate HaX-CoNN on NVIDIA Orin, NVIDIA Xavier, and Qualcomm Snapdragon 865 SoCs. Our experimental results indicate that HaX-CoNN minimizes memory contention by up to 45% and can improve latency and total throughput by up to 32% and 29%, respectively, compared to the state-of-the-art approaches.

==> _TODO.tex <==
autonomous safety citations: https://arxiv.org/pdf/2205.03347.pdf

safety: https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9804610


accuracy: https://www.usenix.org/system/files/atc20-bateni.pdf


autonomous latency task.
Shamsa et al. ~\cite{shamsa2019goal} : no DNN
HetSched~\cite{amarnath2021heterogeneity} propose to an meet latency and safety-criticality constraints : NO DNN



https://docs.google.com/spreadsheets/d/1Lq9fN2uBMb6jRhGGbSFSMCPRNmu-G5t-dcuMcobJ9jU/edit?usp=sharing

https://mines0-my.sharepoint.com/:x:/g/personal/ismetdagli_mines_edu/EacB_9GXBZVNpdw_KiZ-jagBMUlahks6WZbzvS-h08Q8yw?e=W6b17l

==> ignore/review_asplos.tex <==


Evaluation platform is too simple to demonstrate the value of the technique`
Your underlying system only has two accelerators: GPU and DLA. This limits the scope of your evaluation.
I strongly suggest evaluating on (simulated) platforms with multiple subaccelerators (similar to what prior works like Herald and MAGMA evaluated)
overall improvement over baselines (Table 6, Table 8) is only a few percent. This shows that the baselines are already quite optimized, so the proposed work is not improving the state of the art significantly.
Scenario 4 explains H2H puts transitions in suboptimal places, but what about memory contention and how much is the penalty? As it stands much of the model and results are matter-of-fact, which does little to educate the reader about the design decisions and tradeoffs.
The system software implementation is quite weak
Lack of real applications and clarity of how schedules are generated
What is the wallclock time to search for a schedule?
Could you include a naive baseline option to your scheduler?
Are there good transition points that aren't after pooling layers? It seems natural to place them there.
there needs to be more discussion on the system software or hardware challenges in DSAs.
is the accelerator cache hierarchy similar?
What is the data transfer bandwidth across SoCs? Is the data transfer bandwidth the same?
are these applications using the same dataset and starting exactly at the same time? What are some application use cases to represent these experiments?
Why does HaX-CoNN only address static scheduling? What happens when this analysis is applied to dynamic scheduling?
I believe that dynamic scheduling for autonomous systems must be addressed. To do this, I suggest either: (a) Creating a version of HaX-CoNN compatible with dynamic scheduling; or (b) If HaX-CoNN is fundamentally incapable of dynamic scheduling, then it must at least be evaluated in comparison with a reasonable state-of-the-art dynamic scheduling scheme for autonomous systems (e.g., RoboRun, mentioned above) as a baseline, looking at the sorts of dynamic environments that autonomous systems are likely to encounter.
Can the model be extended to consider different arrival rates of inputs? Or, are there references to systems that need this form of static scheduling?
I would suggest the authors better motivate the scenarios evaluated.

==> ignore/review_sigmetrics.tex <==
SIGMETRICS '23 (Winter deadline) Paper #163 Reviews and Comments
===========================================================================
Paper #163 Layer-wise Concurrent DNN Execution Characterization and
Scheduling for Heterogeneous System-on-Chips


Review #163A
===========================================================================

Overall merit
-------------
2. Weak reject

Reviewer expertise
------------------
2. Some familiarity

Paper summary
-------------
It is becoming common for a system to have multiple deep neural networks (DNNs) run concurrently.  They may share GPUs, accelerators and memory.  HaX-CoNN is a scheme for scheduling specific layers of different DNNs to run concurrently on separate GPUs and accelerators.  The paper unconvincingly converts a dynamic, stochastic problem into a static constrained optimization problem, with marginal gains.

Strengths
---------
(S1) HaX-CoNN addresses a difficult problem.

(S2) The scheduler is evaluated with real hardware and benchmarks.

(S3) The experimental results show performance prediction with HaX-CoNN is accurate, and better than other schedulers.

Weaknesses
----------
(W1) The formulation massages a dynamic, stochastic problem into a static constrained optimization problem.

(W2) The experiments only run DNN pairs.

(W3) The performance gains are not impressive, and maybe smaller still in a realistic setting (Fig.1, say).

Comments for authors
--------------------
(S1)  Fig.1 gives an example of a system where multiple DNNs run concurrently on a variety of GPUs, accelerators, etc.  HaX-CoNN (Fig.10) employs a layer-to-accelerator mapping to optimally schedule DNN layers for execution on the hardware.  This is a challenging problem since the accelerators are heterogeneous, speed differences can cause some hardware to become idle, there is contention for shared memory, and transition overhead when a DNN shifts layer execution from one hardware to another.  It is formulated as a min-max optimization problem (Sec.3.4, Eqn.10-12).  It requires per-layer profiling (Table 2), blackbox regression (Fig.7) and a slowdown model for memory interference (Fig.4).

(S2) Sec.4 presents experimental results from running HaX-CoNN using 2 commodity SoCs (Table 4). The workload consists of 4 execution scenarios, 2 DNNs each, running 10 commonly used DNN benchmarks (Table 5).

(S3) Table 6 shows that HaX-CoNN is accurate in estimating latency and throughput for the optimal schedule.  Table 7 and Table 9 show that HaX-CoNN has better performance than alternative schedules in the tested scenarios.

(W1) For workloads like the one in Fig.1, one would aspect task arrivals to be stochastic and not synchronized.  However, the problem formulation in this paper assume the concurrent DNNs start synchronously (Fig.3, Fig.9; p17: "The results are passed to the next task in the workload as soon as both DNNs finish processing"), and stop synchronously (p19: "we increase the number of iterations for the faster DNN so that the difference (in execution time) is eliminated").  Sec.4.1 mentions a TensorRT plugin for inter-DNN synchronization (p15), but provide no details.  To allow for desynchronized DNN start times, delays can be added (p14, item(4)), but that may introduce idle time; it is not clear how these delay values in Table 8 can be determined statically (offline).  Since DNN runtimes are in ms (Table 5), while the SMT solver runs in seconds (p14/para2), it does not seem feasible for the static formulation (Sec.3.4) to be instantiated and solved dynamically.

(W2) Sec.1 mentions an autopilot that has 48 DNNs (Sec.1/para1), Sec.4.1 mentions the need for "multi-accelerator synchronization of DNNs" (p15/para3), and Fig.9 illustrates concurrent execution of 3 DNNs; however, the experiments in Sec.4 run only 2 concurrent DNNs.  Fig.1 shows a variety of tasks (p15/para1: "object detection, image recognition, semantic segmentation, pose estimation and depth estimation"); however, the experiments only use image classification DNNs (Table 5).

(W3) In Table 7, it is not clear what "the best baseline" in the comparison refers to since, for example, in Experiment #4, FPS is highest for "GPU only" but Latency is lowest for GPU&DLA.  In Table 9, only 3 DNN-pairs improve both latency and throughput over "the best baseline" by more than 15%.


Other comments: 

* The layer contention prediction in Fig.4 has a crucial slowdown model, but Step 3 (Sec.2.3) just says "Prior work [63] establishes the relationship between two concurrent workloads as requested throughput and external bandwidth, and builds a piece-wise model to represent the slowdown".

* Table 1 assumes familiarity with DNN terminology and notation.

* What is len(DNN)?



Review #163B
===========================================================================

Overall merit
-------------
2. Weak reject

Reviewer expertise
------------------
2. Some familiarity

Paper summary
-------------
The paper investigate the problem of allocating different parts of different DNNs that must be executed simultaneously on different resources of a system with shared memory. The main contribution is noting that shared memory contention among tasks running on different resources can slowdown the execution, as well as reallocating a task from one resource to another (due to memory transfer). The paper proposes a framework to estimate such slowdowns and build tasks (group of layers of a DNN). This is used as the input to an optimization problem that finds the optimal schedule according to some objective function. The proposal is empirically evaluated on NVIDIA hardware with different DNNs illustrating the improvements over baselines.
layer-wise slowdown model

Strengths
---------
+ The problem seems interesting: a resource allocation problem at the granularity of groups of layers on systems with shared memory and different computational resources.
+ The paper provides evidence that memory contention and resource transitioning generates slowdowns that must be considered.

Weaknesses
----------
- The paper does not provide a rigorous model for the problem. Indeed, it is a classic resource allocation problem on a set of tasks (with dependency and interference) on a shared memory system with heterogeneous resources.
- The slowdown characterization is relatively naive and not comprehensive, considering the interactions between different resources and different tasks (more than two).
- The algorithm to build the tasks (group of layers) is relatively naive and independent of the problem formulation (optimization).

Comments for authors
--------------------
The paper is interesting and provides concrete evidence that memory contention between tasks running on different resources can be a source of slowdown in such systems, as well as the transition of a task from one resource to another. In hindsight, these two findings are quite intuitive but quantifying them on modern systems with current workloads (DNN layers) is interesting. 

However, the framework provided in the paper to tackle the problem is relatively naive. First, a general (theoretical) problem should be formulated where tasks are groups of layers of a DNN to be executed on a system with shared memory and different resources that have interference and dependency among them (the tasks), beyond pairwise. Note that this paper aims at obtaining a fixed schedule for a set of tasks (that can be determined as part of the optimization). 

In particular, the model to build the slowdowns between tasks is quite naive, considering the empirical slowdown of pairwise interactions of specific DNNs on specific hardware. Moreover, the "model"  (given by the simple Algorithm 1) to build the tasks from layers (group of consecutive layers) is naive. 

Last, it is quite likely that slowdowns due to memory contention depend strongly on the hardware, such that the characterization provided on Table 2 is hardware dependent (as likely as DNN architecture and size). Thus, an important consideration would be to determine such slowdows in a more general and rigorous manner.



Review #163C
===========================================================================

Overall merit
-------------
2. Weak reject

Reviewer expertise
------------------
2. Some familiarity

Paper summary
-------------
Multiple concurrently running neural network inference workloads on 
different domain specific accelerators (DSAs) of a mobile/autonomous system 
suffers shared memory contention. Traditional memory subsystem is designed 
to accommodate the memory demands for a processing unit when it runs alone.   
Existing works cannot achieve the optimal execution where the notion of optimality 
is provided in this current paper. This paper proposes HaX-CoNN which is centered 
around characterizing common layers in DNNS according to their DSA-specific 
performance and how they are affected by the shared memory contention. 
Specifically, the layers and DSA mappings are determined by an optimization problem 
that the authors formulated in Section 3.4. HaX-CoNN tries to solve this optimization 
problem via a SAT solver.

Strengths
---------
+ Practically relevant problem 
+ interesting ideas on considering memory contention 
+ the scheduling method is principled
+ comprehensive methodology + experiments

Weaknesses
----------
- Writing clarity needs improvement: It is great that the authors provided sufficiently many 
details to support their claims and to explain their observations. Nevertheless, possibly due 
to the added details, some parts of their writing turn out to be unclear. For example, the 
motivating case study in the introduction appears to be out of place and interrupts the 
reading flow of the introduction. Maybe the authors can move this case study to a later place. 
Another example is the introduction of "optimal transition- and contention-aware assignment 
of layers...". Maybe the authors can think about adding a pointer to the sections that formally 
present this assignment method?  Also, the authors can check the use of the term 
"optimal layer-level scheduling explained..." because this method is only mentioned without 
providing much details.  

-  unclear computation complexity. Solving the optimization involved appears to be computationally  heavy, might even be NP-complete. Though the authors commented on this point on page 14,  to make the comments more convincing, it would be very helpful if the authors can provide  verifiable references. On page 15, the authors mentioned that 10 seconds are needed. I am wondering whether 10 seconds waiting time is affordable for applications on the 
mobile/autonomous systems of interest such as the safety-crucial autonomous vehicles.

==> ignore/trash.tex <==
\subsection{Layer-level mapping}
The bandwidth demand for a DNN significantly varies depending on the input size, the number of layers, computation complexity of each layer, activation functions, etc. So, there will be significantly different phases in bandwidth demand throughout the execution of a DNN. %The memory access pattern of a DNN usually changes in different phases. 
Table~\ref{table:characterization} shows an example of GoogleNet profiling. Memory usage by layers vary from 41\% to 77\%. Considering multiple accelerator will be concurrently running on the system with varying resource utilization, the layers must be classified into the groups so that the bandwidth demand at a time interval can be stable and reliable. So, the layer-level granularity, rather than a workload-level granularity, will enable to accurately estimate the contention between accelerators over system resources. Phase detection for a workload~\cite{phase_detect2006} on shared memory architectures studies among various applications domains and it is orthogonal to this work.

